Search for a Dark Higgs Boson Produced in Association with Inelastic Dark Matter at the Belle II Experiment

Inelastic dark matter models that have two dark matter particles and a massive dark photon can reproduce the observed relic dark matter density without violating cosmological limits. The mass splitting between the two dark matter particles $\chi_{1}$ and $\chi_{2}$, with $m(\chi_{2}) > m(\chi_{1})$, is induced by a dark Higgs field and a corresponding dark Higgs boson $h^{\prime}$. We present a search for dark matter in events with two vertices, at least one of which must be displaced from the interaction region, and missing energy. Using a $365\,\mbox{fb}^{-1}$ data sample collected at Belle II, which operates at the SuperKEKB $e^+e^-$ collider, we observe no evidence for a signal. We set upper limits on the product of the production cross section $\sigma\left(e^+e^- \to h^\prime \chi_1 \chi_2\right)$, and the product of branching fractions $\mathcal{B}\left(\chi_2\to\chi_1 e^+ e^-\right)\times\mathcal{B}\left(h^\prime\to x^+x^-\right)$, where $x^+x^-$ indicates $\mu^+\mu^-, \pi^+\pi^-$, or $K^+K^-$, as functions of $h^{\prime}$ mass and lifetime at the level of $10^{-1}\,\mbox{fb}$. We set model-dependent upper limits on the dark Higgs mixing angle at the level of $10^{-5}$ and on the dark photon kinetic mixing parameter at the level of $10^{-3}$. This is the first search for dark Higgs bosons in association with inelastic dark matter.

==> definitions.tex <==
\RequirePackage{xspace}
\RequirePackage{relsize}

\def\belletwo{\mbox{Belle~II}\xspace}

\def\Pe      {\ensuremath{e}\xspace}        
\def\eplus         {\ensuremath{\Pe^+}\xspace}
\def\eminus         {\ensuremath{\Pe^-}\xspace}
\def\epm        {\ensuremath{\Pe^\pm}\xspace}
\def\epem       {\ensuremath{\Pe^+\Pe^-}\xspace}
\def\chione       {\ensuremath{\chi_{1}}\xspace}
\def\chitwo       {\ensuremath{\chi_{2}}\xspace}
\def\dh       {\ensuremath{h^{\prime}\xspace}}
\def\ap       {\ensuremath{A^{\prime\xspace}}}
\def\mdh       {\ensuremath{m(\dh)}\xspace}
\def\map       {\ensuremath{m(\ap)}\xspace}
\def\mchione       {\ensuremath{m(\chi_{1})}\xspace}
\def\mchitwo       {\ensuremath{m(\chi_{2})}\xspace}

\def\FourS {\ensuremath{\Upsilon(4S)}\xspace}
\def\Bmeson       {\ensuremath{B}\xspace}
\def\Bbarmeson    {\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}\xspace}% do NOT use ensuremath here
\def\BBbar   {\ensuremath{\Bmeson\Bbarmeson}\xspace} 

\def\kaon  {\ensuremath{K}\xspace}
\def\KS    {\ensuremath{\kaon^{\rm\scriptstyle 0}_{\rm\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{\kaon^{\rm\scriptstyle 0}_{\rm\scriptscriptstyle L}}\xspace} 

\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}}

\def\lumi{\mbox{365}\xspace}
\def\lumiinvfb{\mbox{365}\,\invfb\xspace}

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

\newcommand{\cm}{\ensuremath{{\mathrm{\,cm}}}\xspace}

\def \prodbf {product of the production cross section $\sigma\left(\epem \to\dh \chione\chitwo\right)$, and the product of branching fractions $\mathcal{B}\left(\chitwo\to\chione\eplus\eminus\right)\times\mathcal{B}\left(\dh\to x^+x^-\right)$}
\def \prodbfmodeldep {product of the production cross section $\sigma\left(\epem \to\dh \chione\chitwo\right)$, and the branching fraction $\mathcal{B}\left(\chitwo\to\chione\eplus\eminus\right)$}

\def \mathprodbf {\ensuremath{\sigma\left(\epem \to\dh \chione\chitwo\right)\times\mathcal{B}\left(\chitwo\to\chione\eplus\eminus\right)\times\mathcal{B}\left(\dh\to x^+x^-\right)}}
\def \mathprodbfmodeldep {\ensuremath{\sigma_\mathrm{prod}\times\mathcal{B}\left(\chitwo\to\chione\eplus\eminus\right)}}

\def \mathprodbfshort {\ensuremath{\sigma_\mathrm{prod}\times\mathcal{B}\left(\chitwo\to\chione\eplus\eminus\right)\times\mathcal{B}\left(\dh\to x^+x^-\right)}
}

